MedAlign: A Clinician-Generated Dataset for Instruction Following with Electronic Medical Records

The ability of large language models (LLMs) to follow natural language instructions with human-level fluency suggests many opportunities in healthcare to reduce administrative burden and improve quality of care. However, evaluating LLMs on realistic text generation tasks for healthcare remains challenging. Existing question answering datasets for electronic health record (EHR) data fail to capture the complexity of information needs and documentation burdens experienced by clinicians. To address these challenges, we introduce MedAlign, a benchmark dataset of 983 natural language instructions for EHR data. MedAlign is curated by 15 clinicians (7 specialities), includes clinician-written reference responses for 303 instructions, and provides 276 longitudinal EHRs for grounding instruction-response pairs. We used MedAlign to evaluate 6 general domain LLMs, having clinicians rank the accuracy and quality of each LLM response. We found high error rates, ranging from 35% (GPT-4) to 68% (MPT-7B-Instruct), and an 8.3% drop in accuracy moving from 32k to 2k context lengths for GPT-4. Finally, we report correlations between clinician rankings and automated natural language generation metrics as a way to rank LLMs without human review. We make MedAlign available under a research data use agreement to enable LLM evaluations on tasks aligned with clinician needs and preferences.

==> 5_security.tex <==
\section{Security, Privacy, and Compliance}

A university institutional review board granted approval for this study, designated under the reference number 57916.
The data utilized in this research adhered to the university's de-identification protocol.
All authors working with the data have individually undergone and successfully completed institutional training in HIPAA and data privacy, prior to their engagement with the de-identified data.
All models fed with de-identified data were either deployed in an in-house HIPAA compliant compute infrastructure or through a HIPAA business associate agreement.

==> tables/average_rank_259.tex <==
\begin{tabular}{llrrrrrrr}
\toprule
 & Token Length & Count & GPT-4 (32k + MR) & GPT-4 (32k) & GPT-4 (2k) & Vicuña-13B (2k) & Vicuña-7B (2k) & MPT-7B-Instruct (2k) \\
Quartiles &  &  &  &  &  &  &  &  \\
\midrule
1 & 9390-40139  & 68 & 2.721 & 2.537 & 3.162 & 3.890 & 3.904 & 4.787 \\
2 & 40139-65328  & 64 & 2.859 & 2.266 & 3.219 & 4.188 & 3.969 & 4.500 \\
3 & 65328-114779  & 65 & 2.877 & 2.615 & 2.815 & 3.900 & 4.008 & 4.785 \\
4 & 114779-496148  & 62 & 2.895 & 2.250 & 3.290 & 4.097 & 4.113 & 4.355 \\
\midrule
Total &  & 259 & 2.836 & 2.421 & 3.120 & 4.015 & 3.996 & 4.612 \\
\bottomrule
\end{tabular}

